Common-Sense Bias Modeling for Classification Tasks

Machine learning model bias can arise from dataset composition: correlated sensitive features can distort the downstream classification model's decision boundary and lead to performance differences along these features. Existing de-biasing works tackle the most prominent bias features, such as colors of digits or background of animals. However, real-world datasets often include a large number of feature correlations that intrinsically manifest in the data as common sense information. Such spurious visual cues can further reduce model robustness. Thus, domain practitioners desire a comprehensive understanding of correlations and the flexibility to address relevant biases. To this end, we propose a novel framework to extract comprehensive biases in image datasets based on textual descriptions, a common sense-rich modality. Specifically, features are constructed by clustering noun phrase embeddings with similar semantics. The presence of each feature across the dataset is inferred, and their co-occurrence statistics are measured, with spurious correlations optionally examined by a human-in-the-loop module. Downstream experiments show that our method uncovers novel model biases in multiple image benchmark datasets. Furthermore, the discovered bias can be mitigated by simple data re-weighting to de-correlate the features, outperforming state-of-the-art unsupervised bias mitigation methods.

==> 04.method_old.tex <==



\section{Method}
\label{sec:method}



In this section, we propose a novel \textbf{C}ommon-\textbf{S}ense \textbf{B}ias \textbf{D}iscovery method, referred to as CSBD. 
Given a corpus of (image, text description) pairs, our method analyzes pairwise feature correlations based on \textit{common-sense} text descriptions. This is followed by a human-in-the-loop step, where a domain expert reviews the identified correlations and selects the ones that may negatively impact the downstream classification task. Finally, based on the selected correlations, we mitigate model bias via a simple data re-weighting strategy, without a requirement for sensitive group labels. The method is illustrated in Figure~\ref{fig:overview}, with algorithm steps detailed in Algorithm~\ref{algo:b}, and the major components are described below.

% Language-inferred feature distribution
% Discovering feature correlations
% Bias mitigation via re-weighting



\paragraph{Language-inferred feature distribution.} The natural language image descriptions must first be broken down to align with local visual features. We use SceneGraphParser~\cite{wu2019unified} on the text descriptions to split the sentences and extract spans of noun phrases as semantic rich components, e.g. split ``\texttt{The girl has a big smile}'' into ``\texttt{The girl}'' and ``\texttt{a big smile}''. $M$ denotes the the total number of parsed phrases in a dataset. We then use a pre-trained model, Universal Sentence Encoder (USE)~\cite{cer2018universal}, to encode the phrases into embedding vectors;  this model is trained to extract sentence-level embeddings, and performed better than other language models such as CLIP in our experiments (Sec.~\ref{sec:ablation}). 
Phrase vector dimensions are reduced to dimension $d$ (tuneable hyper-parameter) using PCA~\cite{jolliffe2002principal} before being clustered.\looseness=-1

Next, we implement a two stage clustering process, using the K-means clustering algorithm~\cite{lloyd1982least} for both stages: (1) All phrase embedding vectors 
$\boldsymbol{A} \in \mathbb{R}^{d}$ are clustered into $C$ categories, where $C$ is a tunable hyper-parameter (datasets including more diverse categories of objects should have a larger $C$); (2) Each category cluster $c$ is further clustered into $F_c$ features,\footnote{ ``Feature'' in this work refers to a cluster of semantically similar phrases, where the individual phrases (e.g.  ``\texttt{beaming smile}'' and ``\texttt{wide smile}'') are considered interchangeable.}
% We use ``feature'' to refer to a cluster of phrases  
% which are close in embedding space and have similar semantics. They are interchangeable for counting feature distribution.
e.g., if the cluster is for Smile category and $F_c=3$, example features could be ``\texttt{a mild smile}'', ``\texttt{no smile}'', and ``\texttt{beaming smile}''. The value of $F_c$ is determined on a per-cluster basis as follows: we set a pre-defined upper bound ${\sigma}_{max}$, and for each category cluster $c$ we take $F_c$ to be the smallest integer such that the mean within-cluster variance of the features is lower than $\sigma_{max}$. The within-cluster variance of a feature is given by the sum of the squared distance between the centroid point and each point of the cluster; this is the standard measure of spread used in K-means clustering. Using the variance instead of a fixed number of clusters for the second clustering allows each category to contain different number of features; this is important because some categories can have a natural binary split (e.g. eyeglasses/no eyeglasses) while others may have a much wider range of features (e.g. age groups). As a result, we obtain a hierarchy of visual feature descriptions that comprehensively cover the dataset and are consistent with common-sense descriptions. %is perceived with human knowledge. 


\setlength{\textfloatsep}{12pt}
\begin{algorithm}[ht]
\footnotesize
\newcommand{\vect}{\ensuremath{\mathbf{##1}}}

\text{\break}

\textbf{Input:} Image corpus $G = \{g_1, g_2, ..., g_N\}$. \\
\quad \quad \quad Description corpus $D = \{d_1, d_2, ..., d_N\}$ \\

\textbf{Parsing and encoding:}   \\

\quad $D \rightarrow P = \{p_1, p_2, ..., p_M\}$ \quad  \quad $\triangleright$ $P$ is the phrase set  \\

\quad $\boldsymbol{A} = e(P)  = \{ \boldsymbol{p}_1, \boldsymbol{p}_2, ..., \boldsymbol{p}_M \} \in \mathbb{R}^{M\times 512} $  \\


\quad \quad \quad \quad \quad \quad \quad \quad \quad \quad $\triangleright$ $e$ is a pre-trained text encoder \\

\textbf{Clustering:}   \\

\quad  $\boldsymbol{A} \rightarrow C \text{ sets } \{\boldsymbol{S}_1, ..., \boldsymbol{S}_C\}$ \text{\break} \text{\break} \quad \quad \quad \quad $\triangleright$  Vector cluster \\

\quad  $A \rightarrow \{S_1, ..., S_C\}$ \quad 
 $\triangleright$ Natural language phrase cluster  \\

\quad \textbf{for} $c$ from $1$ to $C$ \textbf{do}: \\

\quad \quad $\boldsymbol{S_c} \rightarrow F_c \text{ sets } \{\boldsymbol{B}_1, ..., \boldsymbol{B}_{F_c}\}$, s.t. $\text{Var } \boldsymbol{B}_i \le {\sigma}_{max}$ \\

\quad \quad $S_c \rightarrow \{B_1, ..., B_{F_c}\} $ \\

\quad  $F = F_1 + F_2 + .. + F_C$ \text{\break} \text{\break} $\triangleright$  Number of feature clusters \\

\textbf{Computing correlation:}   \\

\quad \textbf{for} $f$ from $1$ to $F$ \textbf{do}: \\

\quad \quad $\boldsymbol{t}_f = \{t_1, t_2, ..., t_N\}$ \text{\break} \text{\break} \quad $\triangleright$  Feature one-hot indicator \\

\quad \quad , where $t_i = 1$ , if $ \exists \text{\break} p \in B_f $:   $p $ in $d_i$, else $t_i = 0$ \\

\quad \textbf{for} $f$ from $1$ to $F$ \textbf{do}: \\

\quad \quad \textbf{for} $f'$ from $1$ to $F$, $f' \neq f$ \textbf{do}: \\

\quad \quad \quad $\boldsymbol{t}_{f}, \boldsymbol{t}_{f'} \rightarrow \phi_{\boldsymbol{t}_{f}\boldsymbol{t}_{f'}} $  \quad \quad $\triangleright$  phi correlation coefficient \\



\textbf{Outputs:} $[ B_{f}, B_{f'} ]$ , for $f, f'$ where $ \lvert \phi_{\boldsymbol{t}_{f}\boldsymbol{t}_{f'}} \lvert > z $ 

\text{\break}
 \caption{\footnotesize{CSBD. $N$ is the size of the dataset. $M$ is the number of parsed phrases. $C$ is the number of category clusters. ${\sigma}_{max}$ is the upper bound of within-cluster variance. $z$ is the threshold of feature correlation coefficient.} }
\label{algo:b}
\end{algorithm}
\vspace{-5mm}



%https://docs.google.com/drawings/d/1oLBtGZSUBdSc41wPJSlQynTyXwl_SfQFm2A6nr99Hpc/edit
\begin{figure*}[!htbp]
  \centering
\includegraphics[width=0.94\linewidth]{figures/Correlation.pdf}
    \vspace{-2mm}
    \caption{Examples of discovered correlations in CelebA (Left) and MS-COCO (Right) dataset, and the correlation coefficients. Sensitive correlations are circled in yellow, such as ``\texttt{the lady}'' and ``\texttt{smiling}''. The others are viewed as benign, like ``\texttt{man}'' and ``\texttt{mustache}''.
    }
  \label{fig:correlation}
\end{figure*}
\vspace{-2mm}


\paragraph{Discovering feature correlations.} Having extracted a set of feature clusters in the previous step, the next step is understanding feature co-occurence within the dataset. This allows us to identify spurious correlations relevant to the target task, which may cause model bias. 
% \gb{We assume a target task is pre-defined, on which image features that spuriously correlated to target attributes can result in biased model performance}. 
To quantify such correlations: first, we generate a one-hot indicator for each feature: $\boldsymbol{t}_{f} = [t_1, t_2, ..., t_N]$,  where $N$ is the size of the dataset, and $t_i=1$ if the $f^{th}$ feature occurs in the $i^{th}$ image's description, otherwise $t_i=0$. Second, the phi coefficient $\phi$ \cite[p. 282]{Cramr1946MathematicalMO}\footnote{Also known as the Matthews correlation coefficient \cite{Matthews1975ComparisonOT}.}  is used to measure the association between every two indicators. The phi coefficient between two indicators $\boldsymbol{t}_f$ and $\boldsymbol{t}_{f'}$ is defined as follows:
%\footnote{$\neg$ means element-wise ``not''}
\begin{equation}\label{eq:phi def}
\small
\phi_{\boldsymbol{t}_{f}\boldsymbol{t}_{f'}} = \frac{x_{11}x_{00} - x_{10}x_{01}}{\sqrt{x_{1*}x_{0*}x_{*0}x_{*1}}},
\end{equation}
where $c \in [0, C)$, $f, f'\in [0, F_c]$, and
\begin{gather*}
\small
x_{11} = \|\boldsymbol{t}_{f} \cdot \boldsymbol{t}_{f'}\|_1, \quad 
x_{01} = \|(\neg \boldsymbol{t}_{f}) \cdot \boldsymbol{t}_{f'}\|_1, \\
\small
x_{10} = \|\boldsymbol{t}_{f} \cdot (\neg \boldsymbol{t}_{f'})\|_1, \quad
x_{00} = \|(\neg \boldsymbol{t}_{f}) \cdot (\neg \boldsymbol{t}_{f'})\|_1,\\
\small
x_{1*} = \|\boldsymbol{t}_{f}\|_1, \quad x_{0*} = \|\neg \boldsymbol{t}_{f}\|_1, \\ 
\small
x_{*0} = \|\neg \boldsymbol{t}_{f'}\|_1, \quad x_{*1} = \|\boldsymbol{t}_{f'}\|_1.
\end{gather*} 
$\neg$ denotes element-wise negation, $\| \cdot \|_1$ denotes the $L^1$ norm.

Two features are positively correlated (likely to co-occur in an image) if $\phi$ is a positive value, and are negatively correlated (rarely co-occur) if $\phi$ is a negative value. A $\phi$ near zero indicates two features which co-occur randomly. 
% With the generated concept-feature hierarchy, we aim to discover \textit{sensitive feature correlations which affect task prediction}. First, we quantify model prediction's sensitivity to each feature's presence thus the task relevance, denoted as $S_{cf}$. The approach is to learn an activation vector for visual patterns of the feature, and use prediction's derivative with respect to directional change along the vector as sensitivity~\cite{kim2018interpretability}. The concept which has features with maximum sensitivity $\underset{c\in [0,C), f\in [0,F_c)}{max}S_{cf}$ is identified as the target concept $c'$ and it includes $F_{c'}$ target features. 
% % and the concepts model predictions are not sensitive to ($S_{cf} < \mu$) are excluded from the following analysis. 
% To analyze co-occurrence distribution between each target feature and other features, we compute phi coefficient ($\phi$) to measure association for indicators as:

Intuitively, features that have high correlation with any target features can become shortcuts for model learning and cause biased decision-making toward certain subgroups~\cite{tian2022image, brown2023detecting}. Thus feature pairs which have $\lvert \phi \rvert > z$ (where $z$ is an empirically decided threshold and can be adjusted) are returned for examination by a human. The human has access to the common-sense text descriptions of each feature.
% As an example, the feature hierarchy and correlations discovered with threshold $z=0.05$ on CelebA dataset~\cite{jiang2021talk} is shown in Figure.
In most cases, the returned feature pairs are naturally connected (e.g. ``\texttt{teeth visible}'' with ``\texttt{a smile}'', and most facial features with ``\texttt{the face}''). These correlations are usually robust and generalizable, and thus viewed as benign. 
% zee: todo
The benign correlations usually exist, besides, the function of feature correlations vary across different downstream learning scenarios and not all correlations need to be treated. Therefore, a human-in-the-loop step is necessary to ensure that only sensitive correlations that may affect the target task are selected. 
% Due to the presence of these benign correlations, and considering that the function of feature correlations vary across different downstream learning scenarios and not all correlations need to be treated, we include this human-in-the-loop step to ensure that only sensitive correlations that may affect the target task are selected. 
The human-in-the-loop component of our pipeline, like previous efforts~\cite{manjunatha2019explicit, li2021discover, wu2023discover, zhang2023diagnosing}, allows flexibility and transparency for bias mitigation.

% % \textbf{Augmenting to balance}
% \paragraph{Human-in-the-loop Bias Cluster Selection}
% \tocite other methods that have HIL bias migitation efforts.
\paragraph{Bias mitigation via re-weighting.} Enhancing model learning of discounted samples is a common bias reduction approach ~\cite{ahn2022mitigating, sharma2020data, wang2020towards}. Therefore, to simplify the intervention needed for correcting biases surfaced by our method, we follow the previous work in \cite{ahn2022mitigating} to adjust data sampling weights.

Specifically: given a set of targets and human-identified sensitive features correlated to them,\footnote{We use the term ``sensitive features'' to reflect the fact that the primary biases of interest in bias mitigation methods often relate to features such as race/gender/disability/sexuality/etc; however, as we see in Sec.~\ref{sec:experiments}, our method is flexible enough to capture more unexpected types of spurious correlation as well, e.g. ``\texttt{cat}'' and ``\texttt{couch}'' in the MS-COCO dataset.} the goal is to \textit{balance the distribution of samples with vs. without each sensitive feature across the targets}. That is, if the downstream task is smile detection then images with, say, the ``\texttt{man}'' feature and without the feature should have the same ratio of positive to negative target labels. This condition ensures a statistical independence between each feature and target~\cite{qraitem2023bias}.

The new data sampling weights are calculated as follows. We denote the dataset as $D$, target set as $Y$, target feature indicators obtained from the last step as 
$\boldsymbol{t}_{Y} = \{\boldsymbol{t}_{y} : y \in Y\}$, and the sensitive features indicator as $\boldsymbol{t}_{s}$. 
Further, we denote the original feature distribution  with respect to the targets as  $P_D(\boldsymbol{t}_{s}|\boldsymbol{t}_{Y})$ and $ P_{D}(\neg \boldsymbol{t}_{s} | \boldsymbol{t}_{Y})$, with $P$ representing probability. The sampling weight $W (\boldsymbol{t}_{s} | \boldsymbol{t}_{Y})$ for images with feature $s$ across the targets is defined by the following equation:
\begin{equation}\label{eq:sample reweighting}
    P_D(\boldsymbol{t}_{s}| \boldsymbol{t}_{Y})  \cdot W (\boldsymbol{t}_{s} | \boldsymbol{t}_{Y}) = P_{D}(\neg \boldsymbol{t}_{s} | \boldsymbol{t}_{Y})
\end{equation}
In the ideal case where the dataset target feature distribution is already balanced w.r.t the sensitive feature, the sampling weight $W (\boldsymbol{t}_{s} | \boldsymbol{t}_{Y})$ would be equal to 1. The intervention is to treat one sensitive feature $s$ and model bias it causes.

Finally, we also implement randomized augmentations alongside the sampling weights to introduce data diversity. 

% More details for weight setting are in the supplementary.

% sampling probabilities are set based on co-occurrence statistics $x_{11}, x_{00}, x_{10}, \text{and } x_{01}$ obtained from the last step.

% For the $f'^{th}$ target feature, We denote the sampling probability of images including the $f^{th}$ feature of the $c^{th}$ concept as $p_{cf}$, and it is computed based on
% the count of co-occurrence observations $x_{11}$ as below:
% \begin{equation}
% \small
% p_{cf}(x_{11}) = (1 - \frac{x_{11_{cf}}}{\sum_{c\in[0, F_C)} x_{11_{cf}}}) / max(p_{cf}(x_{11}) \text{ for } c\in[0, F_C)).
% \end{equation}





==> 05.results_old.tex <==


\section{Experiments}
\label{sec:experiments}


\begin{table*}[!htbp]
  \small
  \begin{center}
    \setlength{\tabcolsep}{3pt}
    \scalebox{0.84}{
    \begin{tabular}{*{13}{c}}
        \toprule
                  & \multicolumn{2}{c}{Vanilla (no mitigation)} & 
                  \multicolumn{2}{c}{LfF~\cite{nam2020learning}} & \multicolumn{2}{c}{DebiAN~\cite{li2022discover}} &
                  \multicolumn{2}{c}{PGD~\cite{ahn2022mitigating}} &
                  \multicolumn{2}{c}
                  {BPA~\cite{seo2022unsupervised}} &
                  \multicolumn{2}{c}{CSBD (ours)} \\
                  \cmidrule(lr){2-3}
                  \cmidrule(lr){4-5}
                  \cmidrule(lr){6-7}
                  \cmidrule(lr){8-9}
                  \cmidrule(lr){10-11}
                  \cmidrule(lr){12-13}
                   Target & Worst ($\uparrow$)& Avg. ($\uparrow$)& Worst ($\uparrow$) & Avg. ($\uparrow$) & Worst ($\uparrow$) & Avg.($\uparrow$) & Worst($\uparrow$) & Avg. ($\uparrow$) &
                  Worst ($\uparrow$) & Avg. ($\uparrow$) &
                  Worst ($\uparrow$) & Avg.($\uparrow$) \\
        \midrule
        \midrule
                   Smiling  & 0.894 \scriptsize{(3e-3)} & \textbf{0.919} \scriptsize{(2e-3)} & 0.730 \scriptsize{(0.03)} & 0.841 \scriptsize{(7e-3)} & 0.895 \scriptsize{(0.01)} & 0.916 \scriptsize{(7e-3)} & 0.888 \scriptsize{(0.02)}  & 0.917 \scriptsize{(1e-3)} & \underline{0.899}  \scriptsize{(3e-3)} & 0.912 \scriptsize{(6e-3)} & \textbf{0.908} \scriptsize{(3e-3)} & \underline{0.918} \scriptsize{(9e-4)}     \\
           Eyeglasses   & 0.926 \scriptsize{(3e-4)} & \underline{0.964} \scriptsize{(2e-3)}   &  0.810 \scriptsize{(0.02)}  & 0.911 \scriptsize{(7e-3)} & 0.928 \scriptsize{(0.01)} & \underline{0.964} \scriptsize{(6e-3)} & 0.917 \scriptsize{(8e-3)} & 0.960 \scriptsize{(3e-3)}    & \underline{0.929} \scriptsize{(5e-3)} & 0.962 \scriptsize{(2e-3)} &  \textbf{0.938} \scriptsize{(2e-3)} & \textbf{0.965} \scriptsize{(1e-3)}  \\ 

        \bottomrule \\
    \end{tabular}}
    \vspace{-5mm}
    \caption{Treating common-sense bias discovered by CSBD towards the target ground truth label (Target): (1) ``Smiling" and (2) ``Eyeglasses", among the sensitive group label: ``Male" and others, on \textbf{CelebA} dataset. The average classification accuracy of all target-sensitive groups (Avg.), and the worst performing group (Worst), are reported. Results are based on three independent runs and standard deviation is given in parenthesis. The best results are marked in \textbf{bold} and the second best results are \underline{underlined}. Group-level results are in the Supplementary.}
    \vspace{-3mm}
    \label{tab:table1}
  \end{center}
\end{table*}



\begin{table*}[!htbp]
  \small
  \begin{center}
    \setlength{\tabcolsep}{2.6pt}
    \scalebox{0.8}{
    \begin{tabular}{*{14}{c}}
        \toprule
                  & & \multicolumn{2}{c}{Vanilla (no mitigation)} & 
                  \multicolumn{2}{c}{LfF~\cite{nam2020learning}} & \multicolumn{2}
                  {c}{DebiAN~\cite{li2022discover}} & \multicolumn{2}{c}{PGD~\cite{ahn2022mitigating}} &
                  \multicolumn{2}{c}
                  {BPA~\cite{seo2022unsupervised}} &
                  \multicolumn{2}{c}{CSBD (ours)} \\
                  \cmidrule(lr){3-4}
                  \cmidrule(lr){5-6}
                  \cmidrule(lr){7-8}
                  \cmidrule(lr){9-10}
                  \cmidrule(lr){11-12}
                  \cmidrule(lr){13-14}
                   Target & Sensitive & Worst($\uparrow$) & Avg. ($\uparrow$) & Worst ($\uparrow$) & Avg. ($\uparrow$) & Worst ($\uparrow$) & Avg. ($\uparrow$) & Worst ($\uparrow$) & Avg. ($\uparrow$) & Worst ($\uparrow$) & Avg. ($\uparrow$) 
                   & Worst ($\uparrow$) & Avg. ($\uparrow$) \\
        \midrule
        \midrule
             Cat   & Couch & 0.849 \scriptsize{(0.04)} & 0.935 \scriptsize{(8e-3)} & 0.800 \scriptsize{(0.04)} & 0.916 \scriptsize{(0.01)} & 0.821 \scriptsize{(0.01)} & 0.902 \scriptsize{(9e-3)} &  \underline{0.884} \scriptsize{(9e-3)} & \underline{0.940} \scriptsize{(3e-3)} & 0.853 \scriptsize{(0.03)} & 0.925 \scriptsize{(5e-3)}  & \textbf{0.906} \scriptsize{(4e-3)} & \textbf{0.941} \scriptsize{(3e-3)} \\
              Cat   & Keyboard &  \underline{0.948} \scriptsize{(1e-3)} & 0.972 \scriptsize{(6e-3)} & 0.870 \scriptsize{(0.04)} & 0.938 \scriptsize{(9e-3)} & 0.917 \scriptsize{(4e-3)} & 0.949 \scriptsize{(2e-3)} & 0.947 \scriptsize{(7e-4)} & \textbf{0.977} \scriptsize{(2e-4)} & 0.890 \scriptsize{(0.05)} & 0.952 \scriptsize{(0.02} & \textbf{0.953} \scriptsize{(1e-3)} & \underline{0.976} \scriptsize{(6e-4)} \\
             Dog  &  Frisbee & \underline{0.883} \scriptsize{(9e-3)} & 0.927 \scriptsize{(6e-3)} & 0.821 \scriptsize{(0.04)} & 0.893 \scriptsize{(0.02)} & 0.845 \scriptsize{(0.02)} & 0.895 \scriptsize{(2e-3)} & 0.872 \scriptsize{(6e-3)}  & \textbf{0.940} \scriptsize{(4e-3)} & 0.854 \scriptsize{(0.02)} & 0.905 \scriptsize{8e-3)} & \textbf{0.903} \scriptsize{(5e-3)} & \underline{0.934} \scriptsize{(5e-3)} \\
           TV  & Chair & 0.726 \scriptsize{(8e-3)} & 0.893 \scriptsize{(2e-3)} & 0.690 \scriptsize{(0.02)} & 0.867 \scriptsize{(6e-3)} & 0.718 \scriptsize{(0.01)} & 0.876 \scriptsize{(3e-3)} & \underline{0.821} \scriptsize{(7e-3)}  &  \underline{0.907} \scriptsize{(2e-3)} & 0.758 \scriptsize{(0.02)}  &  0.887 \scriptsize{(5e-3)} &  \textbf{0.842} \scriptsize{(7e-3)} & \textbf{0.911} \scriptsize{(1e-3)} \\
            Umbrella & Person & 0.761 \scriptsize{(0.01)} & 0.880 \scriptsize{(2e-3)} & 0.771 \scriptsize{(4e-3)} & 0.854 \scriptsize{(5e-3)} & 0.716 \scriptsize{(0.04)} & 0.857 \scriptsize{(0.01)} &  0.763 \scriptsize{(0.01)}  & \underline{0.887} \scriptsize{(2e-3)} &  \underline{0.777} \scriptsize{(0.02)} & 0.878 \scriptsize{(8e-3)}  & \textbf{0.814} \scriptsize{(9e-3)} & \textbf{0.892} \scriptsize{(1e-3)}\\
            Kite & Person & 0.937 \scriptsize{(0)} & \textbf{0.963} \scriptsize{(4e-4)} & 0.854 \scriptsize{(0.02)} & 0.923 \scriptsize{(7e-3)}  & \underline{0.941} \scriptsize{(0.02)} & \underline{0.960} \scriptsize{(6e-3)} &   0.917 \scriptsize{(0)} & 0.955 \scriptsize{(1e-3)} & 0.921 \scriptsize{(6e-3)} & 0.957 \scriptsize{(2e-3)}  & \textbf{0.945} \scriptsize{(7e-3)} & \underline{0.960}  \scriptsize{(3e-3)} \\


        \bottomrule \\
    \end{tabular}}
    \vspace{-4mm}
    \caption{Treating common-sense bias discovered by CSBD between each target ground truth label (Target) and sensitive group label (Sensitive), for binary object classification task on \textbf{MS-COCO} dataset. The average classification accuracy of all target-sensitive groups (Avg.), and the worst performing group (Worst), resulted from feature correlations, are reported. }
    \vspace{-4mm}
    \label{tab:table2}
  \end{center}
\end{table*}



We conduct downstream experiments to answer: (1) Do the sensitively correlated features reasoned by CSBD align with model bias on popular benchmark datasets? (2) Can prior correlation-robust methods prevent such bias? (3) Is the reasoned bias curable using simple data-wise intervention? 



\subsection{Datasets}
\label{sec:dataset}

\paragraph{CelebA-Dialog}~\cite{jiang2021talk} is a visual-language dataset including captions for images in CelebA~\cite{liu2015deep}, a popular face recognition benchmark dataset containing 40 facial attributes. Each caption describes 5 fine-grained attributes: ``Bangs", ``Eyeglasses", ``Beard", ``Smiling", and ``Age". Since the captions are generated as natural language sentences, they also include other common-sense information like pronouns and people titles (phrases like ``the man'' or ``the lady''). Since we are limited to the facial features each caption describes, our analysis will not pick up the well-known correlations, such as ``HairColor" and ``HeavyMakeUp", studied in prior work~\cite{nam2020learning, zhang2022correct, ahn2022mitigating}; however, we instead identify new correlations not found by other methods (see Sec.~\ref{sec:corr_results}). For classification tasks, we select the target labels as ``Smiling" and ``Eyeglasses", and the sensitive group label to be ``Male'' (here ``label'' refers to the ground truth binary labels). The labels are selected because their corresponding caption-inferred features are discovered by our method to be highly correlated and thus may cause downstream model bias.\looseness=-1
% (Gender is expected to be the sensitive attribute)

\paragraph{MS-COCO 2014}~\cite{lin2014microsoft} is a large-scale scene image datasets including annotations for 80 objects, and each image has 5 descriptive captions generated independently~\cite{chen2015microsoft}. We randomly select 1 caption for each image. Based on our feature correlation analysis, we select 7 target and sensitive label pairs for training downstream models and evaluating bias, as listed in Table~\ref{tab:table2}. For example, we train a model for recognizing ``Dog" and evaluate if the model shows performance disparity for images with/without ``Frisbee".  We perform binary classification on each target label, following ~\cite{wang2023overwriting}. This is because although MS-COCO is more used for multi-label classification, certain labels will need to be treated as auxiliary features in order to reveal their effects on the target and thus study bias caused by feature correlations. 
% It should be noted that the target and sensitive label assignment is not limited to what we experiment on.





\subsection{Implementation}
\label{sec:implementation}

For correlation reasoning, the phrases from the description corpus are encoded to vectors in 512 dimensions using Universal Sentence Encoder (USE). The dimension is reduced using PCA to 30 for the CelebA dataset and 100 for MS-COCO, which ensure that the sum of the PCA components' explained variance was over 90\%. The embedding vectors are then scaled to unit norm before being clustered using K-means. We set the category cluster number $C$ to 8 for CelebA and 50 for MS-COCO. These numbers are empirically selected to ensure no obvious discrepancies in discovered clusters: that is, no redundant clusters or multiple categories in same clusters. For the second step which generates feature clusters, the upper bound of the within-cluster variance $\sigma_{max}$ is set to 0.15 for CelebA and 0.5 for MS-COCO; see Sec.~\ref{sec:ablation} for sensitivity analysis. The threshold $z$ for correlation coefficient between two feature indicators is chosen to be 0.05 (correlation significance is verified by Chi-square test~\cite{Pearson1900}). Empirically, feature correlations higher than $z$ cause bias on the datasets we used. 

% all pair-wise correlations regardless of magnitude will be recorded. (Supplementary)

For the downstream training, we use the same training, validation, and testing split as in \cite{zhang2022correct} for the CelebA dataset, as in \cite{misra2016seeing} on the MS-COCO dataset. 
% zee: todo
However, because of label scarcity of individual objects relative to the entire dataset  (for example, only 3\% of images in MS-COCO contain ``Cat" and 2\% of images contain ``Kite"), to avoid class imbalance problem introducing confounding bias to the classifier, we randomly take subsets of the dataset splits which include 50\% of each target label. Further implementation details are given in the Supplementary.

% Detailed classifier training settings are given in the supplementary material.



% https://docs.google.com/drawings/d/1irdvFDIFwzpOiNwF0t8WOi-f8D9nHXCOOhZKXmQB93U/edit?usp=sharing
\begin{figure*}[!htbp]
  \centering
    \includegraphics[width=1\linewidth]{figures/Embedding-2.pdf}
    \caption{T-SNE results for cat classifiers (``Couch'' as sensitive label) trained with MS-COCO dataset. Target attributes (``Cat" \textcolor{blue}{$\bullet$} \textcolor{orange}{$\bullet$} and ``No cat" \textcolor{green}{$\bullet$} \textcolor{red}{$\bullet$}) are most linearly separable with CSBD-trained embeddings  (E) compared to the baseline and other bias mitigation methods (A-D). Methods which can discover pseudo sensitive groups are marked with group assignment by $\bullet$ and $\times$. Comparing to the real groups (``Couch" \textcolor{red}{$\bullet$} \textcolor{blue}{$\bullet$} and ``No couch" \textcolor{green}{$\bullet$} \textcolor{orange}{$\bullet$}) across which bias is expected to be treated, CSBD obtains the closest estimation.
    }
  \label{fig:embedding}
\end{figure*}


\subsection{Results}
\label{sec:results}

\subsubsection{Correlation discovery results}
\label{sec:corr_results}

\paragraph{CelebA.} Semantic parsing of the image descriptions generates $M=1,\!283,\!552$ phrases for CelebA dataset, and applying CSBD outputs 72 feature pairs that have an absolute correlation coefficient higher than $z=0.05$. By manual check, we determine that the features ``\texttt{smiling}'' and ``\texttt{eyeglasses}'' are both sensitively correlated to people-title features ``\texttt{the man, the guy, ...}'' and ``\texttt{the lady, the girl, ...}'', and we designate other naturally related features like ``\texttt{mouth}'' and ``\texttt{smiling}'' as benign. The correlation values between sensitive features, along with selected benign correlations, are visualized in Figure~\ref{fig:correlation} (Left), and the full list is in the Supplementary. 

\vspace{-3mm}
\paragraph{MS-COCO.} Semantic parsing for descriptions generates 
$M=253,\!467$ phrases. CSBD outputs 220 correlated feature pairs for the MS-COCO dataset. The benign examples include ``\texttt{frisbee}'' and ``\texttt{a game}'', ``\texttt{waves}'' and ``\texttt{ocean}'', etc. The sensitive ones include ``\texttt{cat}'' and ``\texttt{couch}'', ``\texttt{kite}'' and ``\texttt{people}''; see Table~\ref{tab:table2} for the 7 examples chosen for bias mitigation, and the full list is given in the Supplementary. Although these connections are intuitive, models can learn and utilize the feature dependence: for example, recognition of a kite in an image may not be based on its shape but whether it co-occurs with people. Selected results are visualized in Figure~\ref{fig:correlation} (Right).

% The discovered correlations quantify feature distribution imbalance existing in a dataset, which may lead to model bias for the related training tasks. 

\subsubsection{Bias mitigation results}
\label{sec:bias_results}
To verify whether the spurious feature correlations discovered by CSBD can indicate and help mitigate downstream model bias, we report image classification results on CelebA and MS-COCO dataset in Table~\ref{tab:table1} and Table~\ref{tab:table2}.  We use the worst group performance to evaluate model bias, following~\cite{zhang2022correct, ahn2022mitigating, seo2022unsupervised}, and the groups are all combinations of target label and sensitive feature label pairs as in~\cite{zhang2022correct}. Baseline model without bias mitigation (Vanilla) for all tasks presents a gap between the worst-performing group (Worst) and the group average (Avg.), indicating the classifier's bias. For example, images containing Chair but no TV obtain an accuracy of 0.726, 19\% lower than the average accuracy (Table~\ref{tab:table2}). 
% The ``\texttt{tv screen}'' and ``\texttt{chair}'' correlation discovered by our method tells how the sensitive feature affects downstream model decision rule. 
CSBD re-weights sampling probabilities to break the correlations in the dataset, using the reweighting factor given in equation \eqref{eq:sample reweighting}. We see from Tables~\ref{tab:table1} and \ref{tab:table2} that CSBD successfully mitigates model bias (most improved Worst Group Performance) on all targets, outperforming the baseline and other de-biasing methods: LfF~\cite{nam2020learning}, DebiAN~\cite{li2022discover}, PGD~\cite{ahn2022mitigating}, and BPA~\cite{seo2022unsupervised}. Moreover, model classification quality will not be degraded by using our method: CSBD always obtains the highest or the second highest average group accuracy. 



% Differentiate CSBD to feature-based methods: The bias-guiding samples prior approaches identify are noisy; Feature clustering approaches might cluster attributes that have very similar features but very different concepts.


% common-sense feature clusters are  used for sensitive correlation discovery and to re-arrange training sample accordingly. The bias groups in evaluation are split according to dataset ground truth label.




\subsection{Discussion}
\label{sec:discussion}



% No pre-trained model is used but the descriptive text to ground visual features with common sense knowledge. Benefit: flexible emphasis on feature types. Predictable and interpret-able, so avoid extra bias from large models.



We investigate the advantage of our method over other unsupervised bias mitigation methods by discussing the common-sense bias's differentiation to embedding-based bias, specifically, how bias affects model predictions and the treatment required. We visualize image embeddings extracted from the fully connected layer of the ``Cat" classification models trained with MS-COCO\footnote{LfF underperforms the baseline and is included in the Supplementary.}. Model bias can be observed from the vanilla baseline with no intervention (Figure~\ref{fig:embedding} (A)): while target classes are separable for samples without sensitive feature (orange and green dots), for images with sensitive feature the model's prediction boundary for the target is blurred (blue and red dots are partially mixed).  

This is different to the specific bias types our comparison methods study, that sensitive features are easily distinguishable in embedding space. LfF~\cite{nam2020learning} assumes that the biased model presents an unintended decision rule to classify sensitive features, which appear in images aligning with the decision rule. However, this unintended decision rule does not generate in the biased model training (Figure~\ref{fig:embedding} (A)). DebiAN assigns pseudo sensitive groups as two sample splits which get unequal positive prediction rates~\cite{li2022discover}, which cannot capture meaningful feature (Figure~\ref{fig:embedding} (B)).  BPA clusters embeddings and assume different clusters represent different sensitive features~\cite{seo2022unsupervised}. However, embeddings of samples with/without couch feature are not separable and the method only discovers target-related clusters (Figure~\ref{fig:embedding} (D)). PGD does not split pseudo groups but identifies bias conflicting samples by model-computed gradient~\cite{ahn2022mitigating}. Re-weighting based on gradients does not correct the decision boundary (Figure~\ref{fig:embedding} (C)), indicating that samples with the sensitive feature that cause bias are not precisely identified. In sum, for common-sense bias caused by the sensitive features not pronounced in image embeddings, methods which rely only on image will show ineffective bias discovery and mitigation.

In contrast, text-based reasoning provides high-level abstract understanding of the image itself, regardless of how model parameters or embeddings encode the image. Such understanding discovers sensitive features correlated to the target, including ``\texttt{a couch}", precisely. Our method removes the correlation from dataset and trains a model with much clearer decision boundary for ``Cat", not affected by presence of ``Couch" (Figure~\ref{fig:embedding} (E)). Though the reasoning is not based on true feature labels but coarse descriptions with incomplete information (which explains why not all ``Couch" samples are classified in a group), it can still quantify data feature imbalance and lead to effective bias mitigation.

There are other benchmark datasets for bias studies including colored MNIST~\cite{lecun-mnisthandwrittendigit-2010}, corrupted CIFAR~\cite{hendrycks2019benchmarking}, etc. We don not include these datasets because the biases are limited by single feature type (like color), or low-level image properties like brightness and contrast, not in the scope of reasoning features by common-sense knowledge.

% \gb{Discuss: add image feature based bias discovery vs `common-sense' text based bias discovery to justify why our method is better -- while image-based methods rely on only image features, text-based reasoning have high-level abstract understanding of the image itself, which helps discover better cluster.}

% 



% Bias from baseline model (A) and only CSBD discovers thus treats the sensitive feature couch (E).


==> 06.ablation_old.tex <==
\section{Ablation}
\label{sec:ablation}

% \subsection{Method Justification Ablation}



% \begin{table}
% \small
% \begin{center}
% \setlength{\tabcolsep}{4.3pt}
% \scalebox{0.76}{
% \begin{tabular}{ |c|c|c|c|c|c|c|c|c| } 
%  \multicolumn{9}{c}{Text encoder: USE.  Dimension reduction: PCA (Ours)} \\
%  \hline
%   Keyword & C1 & C2 & C3 & C4 & C5  & C6 & C7 & C8 \\ 
%  \hline
%  ``Smile/smiling''  & 0 & \textbf{99.78\%} & 0 & 0 & 0 & 0.22\% & 0 & 0 \\ 
%  \hline
%  ``Eyeglasses'' & 0 & 0 & \textbf{100\%} & 0 &  0& 0 & 0 & 0 \\ 
  
%  \hline
%  ... & \multicolumn{7}{c}{Mean cluster variance ($\downarrow$): 0.3531} & \\
%  \hline
%  \multicolumn{9}{c}{} \\
%  \multicolumn{9}{c}{Text encoder: CLIP.  Dimension reduction: PCA} \\
%  \hline
%  Keyword & C1 & C2 & C3 & C4 & C5 & C6 & C7 & C8 \\ 
%  \hline
%  ``Smile/smiling''  & 0 & 0 & 0.18\% & \textbf{95.67\%} & 4.15\% & 0 & 0 & 0\\ 
%  \hline
%  ``Eyeglasses'' & 0 & 0 & 0 & 0 & \textbf{100\%} & 0 & 0 & 0 \\ 
%  \hline
%  ... & \multicolumn{7}{c}{Mean cluster variance ($\downarrow$): 0.4735} & \\
%  \hline
%  \multicolumn{9}{c}{} \\
%  \multicolumn{9}{c}{Text encoder: USE.  Dimension reduction: UMAP} \\
%  \hline
%  Keyword & C1 & C2 & C3 & C4 & C5 & C6 & C7 & C8 \\ 
%  \hline
%  ``Smile/smiling''  & 0 & \textbf{99.78\%} & 0 & 0 & 0 & 0.22\% & 0 & 0 \\ 
%  \hline
%  ``Eyeglasses'' & 3.6\% & 0 & \textbf{96.4\%} & 0 & 0 & 0 & 0 & 0 \\ 
%  \hline
%  ... & \multicolumn{7}{c}{Mean cluster variance ($\downarrow$): 0.3916} & \\
%  \hline
% \end{tabular}
% }
% \end{center}
% % \vspace{-0.5cm}
% \caption{\label{tab:cluster} The distribution of CelebA description phrases containing ``Smile/smiling'' and ``Eyeglasses'' keywords across 8 clusters (C1-C8). Results are shown for our experiment setting (Top), changing the text encoder to CLIP text encoder (Middle), and changing the dimension reduction technique to nonlinear UMAP (Bottom). } 
% \end{table}




\paragraph{Text-based embedding encoder.} In the language-inferred feature distribution step, we use the Universal Sentence Encoder (USE)~\cite{cer2018universal} which is trained and optimized for sentence level text data. Here we test with a different language model, namely the text encoder of CLIP, which is a modified form of the GPT-2 architecture~\cite{radford2019language}. The encoder is used to extract phrase embeddings, and clustering is performed as described in Algorithm~\ref{algo:b} to generates 8 category clusters on the CelebA dataset. To compare how well different text encoder embeddings retain semantic information to produce reasonable clusters, we compute the mean within-cluster variance of generated clusters. The variance using CLIP text encoder embeddings is 0.4735, while the variance using USE embeddings is 0.3531. Therefore, USE is the better text encoder with respect to clustering common-sense phrases.
% we report the distribution of phrases including ``Smile/smiling'' and ``Eyeglasses'' keywords across all clusters (C1-C8) in Table~\ref{tab:cluster} (the comparison for other category keywords is in the Supplementary). The CLIP text encoder embeddings for ``Eyeglasses'' phrases can be well clustered, but performance for ``Smile/smiling'' clustering is worse than that using USE.  

\vspace{-2mm}
\paragraph{Dimension reduction algorithm.} We experiment with changing the linear dimension reduction technique from PCA~\cite{jolliffe2002principal} to UMAP~\cite{mcinnes2018umap}, which can reflect nonlinear structure from the original embedding space to more than 2 dimensions. Embedding dimension is reduced to 30 to perform clustering as in Sec.~\ref{sec:implementation}.  
% As shown in Table~\ref{tab:cluster}, the clustering result with UMAP is the same as with PCA for ``Smile'' phrases, and is slightly worse for ``Eyeglasses'' phrases. 
The mean within-cluster variance of generated category clusters on the CelebA dataset increases from 0.3531 to 0.3916 when using UMAP, which indicates that the linear dimension reduction PCA applied on embeddings produces better clustering for this application.\looseness=-1



%https://docs.google.com/drawings/d/1RSy967se_Lo68V1f5KqpZJMvtwvUwMFi07oz-9IsAgk/edit?usp=sharing
\begin{figure}[!htbp]
  \centering
    \includegraphics[width=0.94\linewidth]{figures/sensitivity.pdf}
    \caption{Feature clusters generated from 8 categories of CelebA dataset: setting a lower variance threshold $\sigma_{max}$ will generate more clusters, and a uniform threshold is selected for all categories.
    }
  \label{fig:sensitivity}
\end{figure}
\vspace{-5mm}



% Show different Z in Supplementary
\paragraph{Cluster variance threshold.} Feature clusters are obtained by the second clustering on each concept category so that the mean within-cluster variance is lower than a hyper-parameter $\sigma_{max}$. As in Figure~\ref{fig:sensitivity}, the variance decreases and eventually reaches a plateau as feature cluster number increases. Note that different categories present different variance behavior: for example, the Person category includes the single feature ``\texttt{The person}'' so variance is always near zero regardless of partitions. Meanwhile, the Age category includes many more feature varieties such as ``\texttt{the thirties}'', ``\texttt{the eighties}'', ``\texttt{very young}'', etc, so it must be divided into more clusters than other categories before the variance drops below the $\sigma_{max}$ threshold. This demonstrates the necessity of using a variance threshold to set the number of feature clusters on a category-by-category basis rather than choosing one fixed cluster number for all categories.

A reasonable $\sigma_{max}$ is required for our algorithm to discover feature correlations: If $\sigma_{max}$ is too small (for example, at or below the plateau region in Figure~\ref{fig:sensitivity}) then redundant clusters are produced for a same feature, which affects the feature's distribution and thus the correlation measurement. If $\sigma_{max}$ is too large then discrepant features are mixed in a cluster and the cluster's semantic meaning is lost. The effects of applying CSBD with different values of $\sigma_{max}$ on the CelebA dataset is illustrated in Table~\ref{tab:threshold}.

% We quantitatively analyze the sensitivity of CSBD to cluster variance threshold, with respect to bias discovery and mitigation. We test on the Smiling (target)-Gender (sensitive) label pairs as in Table~\ref{tab:table1}. For the discovery, we examine correlations between feature clusters which are related to the target and sensitive label, with varying $\sigma_{max}$. As shown in Table~\ref{tab:threshold}, CSBD returns no highly correlated features for  $\sigma_{max}=0.05, 0.5$. Therefore, no intervention is performed and the model results are same as vanilla baseline. With $\sigma_{max}=0.25, 0.3$, the method discovers the same cluster distribution thus the same setting for bias mitigation.  



\begin{table}[h!]
  \small
  \begin{center}
  \setlength{\tabcolsep}{4.2pt}
    \scalebox{0.74}{
    \begin{tabular}{*{10}{c}}
        \toprule
                 $\sigma_{max}$ & 0.01 & 0.05 & 0.1 & 0.15 & 0.2 & 0.3  \\
        \midrule
        \midrule
                  $\phi$ coefficient & 0.0577 & 0.0651 & 0.105 & 0.106 & 0.0095 & 0.0065    \\
            Worst ($\uparrow$)  & 0.897 \scriptsize{(1e-3)} & 0.901 \scriptsize{(2e-3)} & 0.906 \scriptsize{(5e-3)} & 0.908 \scriptsize{(3e-3)}  & NA & NA    \\
                  Avg. ($\uparrow$) & 0.918 \scriptsize{(5e-4)} & 0.919 \scriptsize{(3e-3)} & 0.918 \scriptsize{(4e-3)} & 0.918 \scriptsize{(9e-4)}  & NA & NA  \\  
        \midrule \\
    \end{tabular}}
    \vspace{-3mm}
    \caption{Sensitivity analysis on variance threshold $\sigma_{max}$ used for splitting feature clusters. $\sigma_{max}$ of 0.1 and 0.15 generate reasonable feature clusters and accurate correlation ($\phi$ coefficient) between ``\texttt{smile}" and ``\texttt{man}" features in CelebA, and show better bias mitigation results (Worst). $\sigma_{max}$ of 0.01 and 0.05 generate redundant clusters that impact correlation measurement thus computed intervention. $\sigma_{max}$ bigger than 0.2 generate clusters with ambiguous semantic meanings so no correlation is discovered (NA). }
    \label{tab:threshold}
  \end{center}
\end{table}
\vspace{-7mm}



% Outputs: Fewer clusters generate broader feature categories. The correlations might change. 




% Ablation: 
% parse into words (no / smile).  We will lose something. 

% 10\% description. 


==> 07.conclusion_old.tex <==
\section{Conclusion and Limitation}
\label{sec:conclusion}

In this work, we for the first time propose to use textural descriptions for systematic bias discovery and mitigation. The approach leads to a new perspective on bias problems and resolves the limitation of latent space based de-biasing which tends to overlook or mis-identify non-dominant features. 
% Instead, descriptions generated using human common-sense reasoning can capture the features, and indicate how their correlation to the target will cause downstream model bias.
Our algorithm applies common-sense reasoning to descriptions generated by humans, which will naturally highlight the features most relevant or noticeable to humans regardless of their size or subtlety in the overall image, and indicates how their correlation to the target will cause downstream bias. Novel sensitive correlations and model biases are discovered for two vision benchmark datasets, and we show state-of-the-art bias mitigation based on the reasoning.
\vspace{-3mm}
\paragraph{Limitations and future work.} First, our method is limited by the availability of text-based descriptions for an image dataset, though we are not dependant on certain description structures or formats in the text. We do not consider leveraging large pre-trained caption generation models and applying CSBD to the synthetic descriptions in this work, due to the risk of introducing new or additional biases from the caption generation models; however, it may be a worthwhile future research direction. Second, we only study pair-wise feature correlations: higher degrees of correlations and how they affect model performance could be explored. Third, our method has not yet been tested on other vision recognition tasks and models, such as object detection and segmentation. However, since the method for discovering sensitive data feature correlations is agnostic to downstream task, this can be a direct next step.\looseness=-1

% The description quality is not required as high as labels and will not break the method. For example, the description for an image with cat and couch could be ``\texttt{The cats are laying together looking very comfortable.}'' which misses the couch feature.


% Future Work: (1) Hybrid image and text feature 



% If text descriptions cover other types of attributes, we could compete. 
